Top-Flavoured Dark Matter in Dark Minimal Flavour Violation

We study a simplified model of top-flavoured dark matter in the framework of Dark Minimal Flavour Violation. In this setup the coupling of the dark matter flavour triplet to right-handed up-type quarks constitutes the only new source of flavour and CP violation. The parameter space of the model is restricted by LHC searches with missing energy final states, by neutral $D$ meson mixing data, by the observed dark matter relic abundance, and by the absence of signal in direct detection experiments. We consider all of these constraints in turn, studying their implications for the allowed parameter space. Imposing the mass limits and coupling benchmarks from collider searches, we then conduct a combined analysis of all the other constraints, revealing their non-trivial interplay. Especially interesting is the combination of direct detection and relic abundance constraints, having a severe impact on the structure of the dark matter coupling matrix. We point out that future bounds from upcoming direct detection experiments, such as XENON1T, XENONnT, LUX-ZEPLIN, and DARWIN, will exclude a large part of the parameter space and push the DM mass to higher values.

==> praeamble/befehle.tex <==
%Lösche voreingestellte Symbole
\savesymbol{a}
\savesymbol{b}
\savesymbol{d}
\savesymbol{e}
\savesymbol{gg}
\savesymbol{k}
\savesymbol{l}
\savesymbol{L}
\savesymbol{p}
\savesymbol{r}
\savesymbol{s}
\savesymbol{t}
\savesymbol{div}
\savesymbol{SS}



%Sprachen
\newcommand{\englisch}[1]{\begin{otherlanguage}{british}#1\end{otherlanguage}}
\newcommand{\deutsch}[1]{\begin{otherlanguage}{ngerman}#1\end{otherlanguage}}

%Textauszeichnung
\newcommand{\schlsswrt}[1]{\textbf{#1}}  %Schlüsselwort
\newcommand{\betont}[1]{\textsl{#1}} % Betonung

%Anzeigestil in Formeln
\newcommand{\D}{\displaystyle}

%Mathematische Funktionen
\DeclareMathOperator{\varRe}{Re}  %Realteil als Re
\DeclareMathOperator{\varIm}{Im}  %Imaginärteil als Im
\DeclareMathOperator{\arcsec}{arcsec} 
\DeclareMathOperator{\arccsc}{arccsc}
\DeclareMathOperator{\arccot}{arccot}
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\arcsech}{arcsech}
\DeclareMathOperator{\arccsch}{arccsch}
\DeclareMathOperator{\arccoth}{arccoth}

\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\div}{div}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\Gl}{GL}
\DeclareMathOperator{\Lie}{Lie}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\diag}{diag}
\newcommand{\ip}{\ \lrcorner\ }

%Mathematische Akzente
\newcommand{\konj}[1]{\overline{#1}}  % komplex Konjugiertes
\newcommand{\evec}[1]{\hat{#1}}  % Einheitsvektoren auszeichnen
\newcommand{\ten}[1]{\overleftrightarrow{#1}}	% Tensorzeichen

%Griechische Buchstaben und co
\newcommand{\a}{\alpha}
\newcommand{\b}{\beta}
\newcommand{\d}{\partial}
\newcommand{\del}{\delta}
\newcommand{\Del}{\Delta}
\newcommand{\e}{\varepsilon}
\newcommand{\g}{\gamma}
\newcommand{\G}{\Gamma}
\newcommand{\k}{\kappa}
\newcommand{\l}{\lambda}
\newcommand{\L}{\Lambda}
\newcommand{\p}{\phi}
\newcommand{\ps}{\psi}
\newcommand{\r}{\rho}
\newcommand{\s}{\sigma}
\newcommand{\t}{\theta}
\newcommand{\A}{\mathcal A}
\newcommand{\Acl}{A_{cl}}
\newcommand{\B}{\mathbf B}

%Farben
\newcommand{\blue}[1]{\color{blue}#1\color{black}}
\newcommand{\red}[1]{\color{red}#1\color{black}}
\newcommand{\green}[1]{\color{green}#1\color{black}}


%Grenzwerte
\newcommand{\limes}[1]{\underset{#1}\lim}  %lim mit Argument darunter
\newcommand{\gw}[1]{\xrightarrow{#1}}  %Pfeil mit Argument darüber (Grenzwert)
\newcommand{\glmgw}[1]{\rightrightarrows} % gleichmäßiger Grenzwert

%Mengen
\newcommand{\N}{\mathbbm{N}}
\newcommand{\Z}{\mathbbm{Z}}
\newcommand{\Q}{\mathbbm{Q}}
\newcommand{\R}{\mathbbm{R}}
\newcommand{\Rpl}{\mathbbm{R}_+}
\newcommand{\Rmin}{\mathbbm{R}_-}
\newcommand{\C}{\mathbbm{C}}
\newcommand{\K}{\mathbbm{K}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\JJ}{\mathcal{J}}
\newcommand{\SS}{\mathcal{S}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\gg}{\mathbf g}


%Matrizen
\newcommand{\mat}[1]{\hat{#1}} % Akzent für Matrizen
\newcommand{\NullMatrix}{\textbf{0}}
\newcommand{\EinsMatrix}{\textbf{1}}

%Bra, Ket-Vaktoren
\newcommand{\bra}[1]{\langle #1 |}
\newcommand{\ket}[1]{| #1 \rangle}

%Operatoren
\newcommand{\diff}[2]{\frac{\text{d}#1}{\text{d}#2}} %Ableitung nach Leibnitz geschrieben
\newcommand{\pdiff}[2]{\frac{\partial#1}{\partial #2}} %partielle Ableitung nach Leibnitz geschrieben
\newcommand{\laplace}{\Delta} % Laplace-Operator


%Einheiten
\usepackage{gensymb} % notwendiges Paket mit Symbolen
\newcommand{\Einheit}[1]{\,\text{#1}}
\newcommand{\Ampere}{\Einheit{A}}
\newcommand{\Sekunde}{\Einheit{s}}
\newcommand{\Gramm}{\Einheit{g}}
\newcommand{\Meter}{\Einheit{m}}
\newcommand{\Newton}{\Einheit{N}}
\newcommand{\Pascal}{\Einheit{Pa}}
\newcommand{\Farad}{\Einheit{F}}
\newcommand{\Volt}{\Einheit{V}}
\newcommand{\Coulomb}{\Einheit{C}}
\newcommand{\Joule}{\Einheit{J}}
\newcommand{\Tesla}{\Einheit{T}}
\newcommand{\Liter}{\Einheit{l}}
\newcommand{\Gauss}{\Einheit{G}}
\newcommand{\Ohm}{\,\ohm}
\newcommand{\Siemens}{\Einheit{S}}
\newcommand{\Henry}{\Einheit{H}}
\newcommand{\Watt}{\Einheit{W}}
\newcommand{\Hertz}{\Einheit{Hz}}
\newcommand{\Grad}{\degree}
\newcommand{\Celsius}{\,\celsius}
\newcommand{\Kelvin}{\Einheit{K}}
\newcommand{\varGrad}{\Einheit{grd}}
\newcommand{\EVolt}{\Einheit{eV}}
\newcommand{\Mol}{\Einheit{mol}}
\newcommand{\Skalenteil}{\Einheit{Skt}}
\newcommand{\Angstroem}{\Einheit{\AA}}

\newcommand{\rpm}{\Einheit{rpm}}
\newcommand{\dalton}{\Einheit{da}}
\newcommand{\molar}{\Einheit{M}}

\newcommand{\Yotta}{\Einheit{Y}\hspace{-0.5ex}}
\newcommand{\Zetta}{\Einheit{Z}\hspace{-0.5ex}}
\newcommand{\Exa}{\Einheit{E}\hspace{-0.5ex}}
\newcommand{\Peta}{\Einheit{P}\hspace{-0.5ex}}
\newcommand{\Tera}{\Einheit{T}\hspace{-0.5ex}}
\newcommand{\Giga}{\Einheit{G}\hspace{-0.5ex}}
\newcommand{\Mega}{\Einheit{M}\hspace{-0.5ex}}
\newcommand{\Kilo}{\Einheit{k}\hspace{-0.5ex}}
\newcommand{\Hekto}{\Einheit{h}\hspace{-0.5ex}}
\newcommand{\Deka}{\Einheit{da}\hspace{-0.5ex}}
\newcommand{\dezi}{\Einheit{d}\hspace{-0.5ex}}
\newcommand{\centi}{\Einheit{c}\hspace{-0.5ex}}
\newcommand{\milli}{\Einheit{m}\hspace{-0.5ex}}
\newcommand{\mikro}{\,\micro\hspace{-0.5ex}}
\newcommand{\nano}{\Einheit{n}\hspace{-0.5ex}}
\newcommand{\pico}{\Einheit{p}\hspace{-0.5ex}}
\newcommand{\femto}{\Einheit{f}\hspace{-0.5ex}}
\newcommand{\atto}{\Einheit{a}\hspace{-0.5ex}}
\newcommand{\zepto}{\Einheit{z}\hspace{-0.5ex}}
\newcommand{\yokto}{\Einheit{y}\hspace{-0.5ex}}


==> praeamble/makros.tex <==
%Leerraum statt Text einfügen
\newlength{\tmplen}
\newcommand{\leer}[1]{\settowidth{\tmplen}{#1}\hspace*{\tmplen}}
\newcommand{\nleer}[1]{\settowidth{\tmplen}{#1}\hspace*{-\tmplen}}

%Definitionsbox:
\newcommand{\mybox}[2]{
    \bigbreak
    \fcolorbox{black}{white}{\parbox{\linewidth}{
    	\textbf{#1} \\
    	#2}}
    \bigbreak
}


==> praeamble/pakete.tex <==
\usepackage[T1]{fontenc}
\usepackage[latin1]{inputenc} %lege Latin1 als Eingabgeformat fest
\usepackage[ngerman,british]{babel} %lege Deutsch als Sprache fest, neue Rechtschreibung
	\addto\captionsngerman{\renewcommand{\figurename}{Abb.}\renewcommand{\tablename}{Tab.}} %eigene Kürzel für Abbildungen und Tabellen
\usepackage{amsmath} %AMS Mathematik-Pakte
\usepackage{amssymb} %AMS Symbol-Paket
\usepackage{mathrsfs} %Skript-Buchstaben
\usepackage{bbm} %für Mengenzeichen
\usepackage{mdwlist} %mehr Listenumgebungen
\usepackage{paralist} %mehr Listenumgebungen
	\setlength{\pltopsep}{0.5em} %Abstand zwischen Liste und umgebenden Text für paralist
	\setlength{\plitemsep}{0.3em} %Abstand zwischen Listenelementen für paralist
\usepackage{array}
\usepackage{graphicx} %zum Einbinden von Grafiken
\usepackage{booktabs} %stellt unterschiedlich dicke horizontale Trennlinien für Tabellen bereit
\usepackage{multirow} %zum Setzen von mehrspaltigen Zellen in Tabellen
\usepackage{multicol}
\usepackage{dcolumn} %zum Setzen reiner Zahlenspalten in Tabellen
\usepackage{wrapfig} %Umgebungen für textumflossene Grafiken
\usepackage{url} %stellt Umgebung zum Setzen von URL bereit
\usepackage{ziffer} %legt Komma statt Punkt als Trennzeichen in Dezimalbrüchen fest
\usepackage{scrpage2} %zu KOMA-Script kompatible Kopf- und Fußzeilen
\usepackage{color} %Unterstützung für Farbe
\usepackage[version=3]{mhchem} %für den Satz Chemischer Formeln
\usepackage{lscape} %Querformat-Umgebung

\usepackage{amsthm,dsfont,mathtools} % Weiteres Mathezeug
\usepackage{savesym} %Zum Überschreiben voreingestellter Befehle

%Für Feynmandiagramme:
\usepackage{latexsym}
\usepackage{feynmp}
